BattVAE-GP: Generative Modeling of Long-Horizon Battery Degradation with Uncertainty Quantification

Long-horizon physics-based simulations of battery degradation provide mechanistic insight but remain computationally expensive, limiting their use for dense exploration of operating conditions over extended cycle life. Here, we propose a hybrid physics-probabilistic learning framework for surrogate modeling of lithium-ion battery degradation trajectories at unseen charging rates. Cycle-resolved degradation data generated with a DFN/P2D electrochemical model in PyBaMM are first transformed into capacity-aligned voltage and derivative features and encoded using a Variational Autoencoder (VAE). The resulting two-dimensional latent space organizes degradation trajectories according to both cycle progression and charging protocol. A sparse multitask Gaussian process (GP) is then trained in this latent space using cycle number and C-rate as input variables, providing continuous interpolation of latent degradation dynamics together with posterior uncertainty estimates. Under protocol-level holdout evaluation, the latent-space GP accurately recovers unseen C-rate trajectories and exhibits uncertainty behavior consistent with the support of the training data. When queried at unseen interior C-rates, the model generates latent trajectories that remain coherently positioned between neighboring simulated protocols. Decoding the GP-predicted latent states through the frozen VAE decoder yields smooth voltage-capacity evolution, while Monte Carlo propagation of the GP latent posterior through an auxiliary latent to State of Health (SOH) predictor provides uncertainty-aware SOH estimates. The proposed BattVAE-GP framework therefore offers a computationally efficient and uncertainty-aware surrogate for long-horizon degradation modeling, providing a structured basis for extending battery health prediction toward richer operating conditions and future simulation-experiment fusion.

==> extra.tex <==

% \section{Methods}
% \subsection{Physics-based modeling} \label{sec:pybamm}
% Physics-based cycling data were generated using PyBaMM (Python Battery Mathematical Modelling) \cite{sulzer2021python}. Simulations were performed with the Doyle–Fuller–Newman (DFN/P2D) model \cite{doyle1995design, doyle1993modeling}, which resolves electrochemical transport and interfacial kinetics in the through-thickness direction of the current collector–negative electrode–separator–positive electrode stack, while neglecting in-plane inhomogeneities. Model parameters were initialized from the O'Kane \textit{et al.} \cite{D2CP00417H} parameter set. In addition, the negative-electrode open-circuit potential (OCP) was overridden using the corresponding function from Chen \textit{et al.} \cite{chen_2020}, i.e., the entry “Negative electrode OCP [V]” in the O'Kane \textit{et al.} parameter values was replaced by the Chen \textit{et al.} OCP, to match the intended negative-electrode thermodynamics.

% PyBaMM provides several thermal submodels that can be coupled to DFN/P2D to obtain thermo-electrochemical simulations. However, for the LG M50T parameterization adopted here, the available literature does not provide a complete set of thermal parameters (e.g., effective thermal conductivities and heat capacities) required to calibrate these models consistently. While entropic (reversible) heating coefficients as functions of stoichiometry have been reported, complementary measurements needed for thermal closure are typically unavailable. Following this limitation, no thermal submodel is enabled in this work and the temperature is assumed constant throughout cycling.

% To represent long-horizon capacity fade under repeated cycling, DFN was augmented via PyBaMM’s options interface with coupled degradation physics. Specifically, SEI growth was enabled using a solvent-diffusion-limited formulation, with SEI-driven porosity change activated. Lithium plating was enabled as partially reversible, with plating-induced porosity change included. Mechanical degradation was represented using PyBaMM’s particle mechanics option with swelling and cracking in one electrode and swelling-only in the other (as specified by the tuple option), and loss of active material (LAM) was modeled as stress-driven, enabling coupling between electrochemical operation, particle mechanics, and capacity loss.

% All simulations were solved using PyBaMM's IDAKLU DAE solver. Relative and absolute tolerances ($r_{tol}=, a_{tol}=$ were provided through the simulation configuration. Spatial discretization used fixed resolution with $x_n=x_s=x_p=10$ points through the negative electrode, separator, and positive electrode domains, and $r_n = r_p = 30$ points in the negative and positive particle domains. 

% Each simulation followed a repeated discharge–rest–charge–rest sequence, designed to (i) standardize the discharged state each cycle and (ii) probe degradation sensitivity to the charging C-rate while keeping the discharge condition fixed:

% \begin{itemize}
%     \item \textbf{Initialization:} cell set to 4.2 V (fully charged state by voltage).
%     \item \textbf{Discharge (CC):} constant-current discharge at 1C down to a cutoff voltage of 2.5 V.
%     \item \textbf{Rest:} open-circuit rest for 30 min, allowing voltage relaxation toward quasi-equilibrium.
%     \item \textbf{Charge (CC):} constant-current charge at a prescribed C-rate until the terminal voltage reaches 4.2 V (no CV hold in the base protocol).
%     \item \textbf{Rest:} open-circuit rest for 30 min.
% \end{itemize}

% This sequence was repeated for 5000 cycles. The protocol was executed for multiple charge rates such as 
% 0.2C, 0.3C, 0.4C, 0.5C, 0.6C, 0.75C, 0.8C, 1.0C while maintaining discharge at 1C for all cases. Hereafter, this set of steps is referred to as the cycling protocol.

% This design focuses the comparison on how increasing charge rate changes electrochemical polarization and associated degradation kinetics, while reducing confounding from discharge conditions. A limitation is that omitting a CV step can alter the upper-SOC dwell time relative to standard CCCV charging; this is intentional here to keep the protocol consistent and to attribute differences primarily to the CC charge rate.

% As aging progresses, the accessible capacity decreases and the charge passed per cycle changes accordingly. To compare degradation trajectories across charging rates on a consistent basis, degradation indicators (e.g., capacity loss, resistance growth, loss of cyclable lithium) were tracked as a function of total charge throughput $Q_{tot}$, defined as:
% \begin{equation}
%     Q_{tot}(t) = \int_0^t |I(\tau)| d\tau
% \end{equation}
% where $∣I(t)∣$ is the magnitude of the applied current. Throughput normalization is particularly useful when different C-rates lead to different polarization and hence different realized capacity per cycle, preventing misleading comparisons based solely on cycle count.

% In addition to throughput-based analysis, per-cycle discharge capacity can be computed directly from the discharge segment by integrating current over the discharge interval, enabling capacity-fade curves over cycles and mapping between cycle index and $Q_{tot}$ .
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{Dataset construction and problem formulation} \label{sec:dataset}
% PyBaMM simulations were logged at a fixed sampling period of 10 s, exporting per-timestep t, V, I, Cycle where t is time in seconds, V is terminal voltage, I is applied current, and Cycle indexes the cycle number. Time-grid sampling leads to rate-dependent sequence lengths (higher C-rate $\rightarrow$ shorter segments). To obtain rate-invariant representations, we convert each cycle to a capacity-parameterized form. Further, for each cycle of particular C-rate data, we compute cumulative capacity via trapezoid-like accumulation on the discrete grid:
% \begin{align}
%     \Delta t_k = t_k - t_{k-1}, \hspace{0.5cm} \Delta Q_k = \dfrac{I_k \Delta t_k}{3600}, \hspace{0.5cm} Q_k = \sum_{j \le k} \Delta Q_j,
% \end{align}
% and then re-zeros per cycle as $Q_k^{cycle} = Q_k - Q_{k0}$, where $k_0$ is the first time-step of that cycle. Moreover, we only consider the charge-discharge part in the cycle. Segment capacities are explicitly re-zeroed at segment start and made monotone increasing (discharge sign-flipped). This yields strictly non-negative, increasing abscissae for both segments, suitable for interpolation.

% Per dataset, we find the maximum effective capacity ($q_0$) i.e. $Q_{max}-Q_{min}$ to obtain a normalization scale. Each cycle is then mapped to a common normalized grid
% \begin{align}
%     q \in [0,1], \hspace{0.5cm} q_n = \dfrac{n}{N-1}, n = 0,...,N-1,
% \end{align}
% where N is the number of interpolation points. The grid is converted back to an absolute Ah grid for interpolation as $Q_{grid}(q) = qq_0$. To ensure charge and discharge share a consistent SOC-like axis (enabling meaningful hysteresis), discharge is "SOC-aligned" using the achieved end-of-charge fraction $q_top$.
% \begin{align}
%     q_top = \dfrac{max(Q_{ch})}{q_0}, \hspace{0.5cm} Q_{ch}^{soc}=Q_{ch}, \hspace{0.5cm} Q_{dis}^{soc}=q_{top}q_0 - Q_{dis} 
% \end{align}
% This constructs charge and discharge curves on a common increasing SOC abscissa.

% Voltage curves are interpolated on $Q_{grid}$ using shape preserving cubinc Hermite interpolant (PCHIP), separately for charge and discharge. Crucially, the implementation also extracts analytic derivatives from the fitted interpolant as $\dfrac{dV(q)}{dQ}$ and $\dfrac{d^2V(q)}{dQ^2}$. We compute the incremental capacity analysis (ICA) using $\dfrac{dQ(q)}{dV} = \dfrac{1}{dV/dQ}$. Further, we compute the hysteresis on the overlap of charge and discharge supports as $H_{raw}(q) = V_{ch}(q) - V_{dis}(q)$. Below figure illustrates all the variables and their evolution.

% %%%%%% PUT THE FIGURE

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{VAE model for degradation trajectories}
% The preprocessing described in Section~\ref{sec:dataset} converts each simulated cycle into a capacity-aligned, multi-channel trajectory \(x \in \mathbb{R}^{C\times N}\) (with validity masks for derivative-like channels). The role of the generative model is twofold: (i) compress these high-dimensional trajectories into a low-dimensional representation that preserves degradation signatures, and (ii) impose a probabilistic structure on this representation so that interpolation and uncertainty-aware generalization across charging rates are well-defined.

% A deterministic autoencoder achieves compression by learning an encoder \(f_\phi(\cdot)\) that maps \(x\) to a latent code \(z\), and a decoder \(g_\theta(\cdot)\) that reconstructs \(\hat{x}=g_\theta(z)\). However, standard autoencoders do not specify a generative process for \(z\): the latent space is not regularized toward a known prior and may contain disconnected regions, which can make sampling and downstream uncertainty handling ambiguous. We therefore adopt a variational autoencoder (VAE)~\cite{kingma2013auto}, which casts representation learning as inference in a latent-variable model.

% In the VAE, latent variables follow a prior \(p(z)\), chosen as an isotropic Gaussian,
% \begin{equation}
% p(z)=\mathcal{N}(0,I),
% \end{equation}
% and observations are generated through the decoder likelihood \(p_\theta(x\mid z)\). The encoder provides an approximate posterior over latents,
% \begin{equation}
% q_\phi(z\mid x)=\mathcal{N}\!\left(\mu_\phi(x),\,\mathrm{diag}(\sigma_\phi^2(x))\right),
% \end{equation}
% with sampling performed via the reparameterization trick,
% \begin{equation}
% z=\mu_\phi(x)+\sigma_\phi(x)\odot\varepsilon,\qquad \varepsilon\sim\mathcal{N}(0,I),
% \end{equation}
% enabling end-to-end optimization by backpropagation.

% Model parameters are learned by maximizing the evidence lower bound (ELBO) on \(\log p_\theta(x)\),
% \begin{equation}
% \log p_\theta(x)\ \ge\ \mathbb{E}_{q_\phi(z\mid x)}\!\left[\log p_\theta(x\mid z)\right]\ -\ \mathrm{KL}\!\left(q_\phi(z\mid x)\,\|\,p(z)\right),
% \end{equation}
% which balances reconstruction fidelity with latent regularization. We minimize the negative ELBO using a \(\beta\)-VAE formulation~\cite{higgins2017betavae},
% \begin{equation}
% \mathcal{L}_{\mathrm{VAE}}(x)=
% -\mathbb{E}_{q_\phi(z\mid x)}\!\left[\log p_\theta(x\mid z)\right]
% +\beta\,\mathrm{KL}\!\left(q_\phi(z\mid x)\,\|\,p(z)\right),
% \end{equation}
% where \(\beta\) controls the trade-off between reconstruction accuracy and latent smoothness/structure. For a diagonal-Gaussian posterior and standard normal prior, the KL divergence admits the closed form
% \begin{equation}
% \mathrm{KL}\!\left(q_\phi(z\mid x)\,\|\,p(z)\right)
% =\frac{1}{2}\sum_{j=1}^{d}\left(\mu_j^2+\sigma_j^2-\log\sigma_j^2-1\right),
% \end{equation}
% with \(d\) the latent dimensionality.

% We model \(p_\theta(x\mid z)\) as an isotropic Gaussian in the observation space, such that the negative log-likelihood reduces (up to constants) to a squared reconstruction error. Because derivative-like channels are only reliable on interior regions of the capacity grid, we apply validity masks \(m\) during training,
% \begin{equation}
% -\log p_\theta(x\mid z)\ \propto\ \lVert m\odot(x-\hat{x})\rVert_2^2,\qquad \hat{x}=g_\theta(z),
% \end{equation}
% ensuring that undefined boundary regions do not bias learning.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.95\linewidth]{figures/VAE.png}
%     \caption{Overview of the VAE used for degradation trajectories. Capacity-aligned multi-channel cycle trajectories $x$ are encoded to a Gaussian posterior $q_\phi(z\mid x)=\mathcal{N}(\mu_\phi(x),\mathrm{diag}(\sigma_\phi^2(x)))$; latent samples are drawn via the reparameterization trick and decoded to reconstruct $\hat{x}$. The latent space is subsequently used for GP regression versus charging C-rate.}
%     \label{fig:vae}
% \end{figure}

% \paragraph{Encoder architecture.}
% Each input sample corresponds to a single cycle represented on the normalized capacity grid \(q\in[0,1]\) as a multi-channel sequence. The encoder operates on voltage-derived signatures extracted for both charge and discharge segments: the voltage curves \(V_{\mathrm{ch}}(q)\) and \(V_{\mathrm{dis}}(q)\), their first derivatives with respect to capacity \(dV_{\mathrm{ch}}/dQ\) and \(dV_{\mathrm{dis}}/dQ\) (differential voltage analysis), their second derivatives \(d^2V_{\mathrm{ch}}/dQ^2\) and \(d^2V_{\mathrm{dis}}/dQ^2\), and the incremental-capacity signals \(dQ/dV\) computed for charge and discharge (incremental capacity analysis). In addition, we include the hysteresis profile \(H(q)=V_{\mathrm{ch}}(q)-V_{\mathrm{dis}}(q)\) as a separate channel. Together, these constitute nine physically motivated channels describing each cycle trajectory. We also include the capacity coordinate \(q\) itself as an input channel to provide an explicit positional reference along the trajectory. To increase the representational capacity for fine-scale structure, \(q\) is further expanded into a low-dimensional Fourier feature embedding~\cite{gao2024h}; specifically, four sinusoidal features of \(q\) are concatenated to the raw channels. The resulting per-token input therefore has \(9\) signal channels plus \(1\) coordinate channel plus \(4\) Fourier features, for a total of \(13\) channels.

% The concatenated sequence is first mapped to a token-wise embedding using a learned linear projection, producing a contextual representation at each capacity grid point. This embedded sequence is then processed by a lightweight Transformer encoder~\cite{vaswani2017attention} consisting of two self-attention layers (rather than the deeper stacks commonly used in machine translation). This design choice reflects the comparatively lower semantic complexity of the present time-series signals while retaining the Transformer's ability to model long-range dependencies along the capacity axis. Each Transformer layer is conditioned on the charging C-rate through feature-wise linear modulation (FiLM)~\cite{perez2018film}, enabling the encoder to adapt its representations as a function of operating condition. Moreover, self-attention naturally accommodates the validity masks introduced during preprocessing: masked regions (which grow in later-life cycles due to shortened CC segments) can be excluded from attention, allowing the encoder to focus on physically meaningful support without introducing artifacts from undefined boundary regions.

% To obtain a fixed-dimensional latent representation, the Transformer output is aggregated using a learned attention-based pooling mechanism~\cite{ilse2018attention}, where a global trainable query attends over valid tokens and produces a weighted sum representation. The pooled representation is passed through a fully connected layer and then projected to the parameters of the approximate posterior, yielding the latent mean and (log-)variance vectors \(\mu_\phi(x)\) and \(\sigma_\phi(x)\) that define \(q_\phi(z\mid x)\).


% \paragraph{Decoder architecture.}
% The decoder reconstructs the cycle-level channels on the common capacity grid while being intentionally lightweight, so that the latent variable \(z\) remains the primary carrier of degradation information rather than being bypassed by an overly expressive generator. Operationally, the decoder implements a neural-field mapping \(\hat{x}(q)=g_\theta(z,q)\) evaluated at the \(N\) points of the capacity grid. For each sample, the latent vector \(z\in\mathbb{R}^d\) is broadcast across the sequence length and concatenated with the Fourier-feature embedding of the capacity coordinate used in the encoder. The concatenated token representation is mapped to a hidden sequence via a learned linear projection and processed by a shallow stack of MLP blocks. No explicit conditioning (e.g., FiLM on C-rate) is applied in the decoder; this design choice discourages reconstruction from relying on protocol-level side information and instead encourages such information to be encoded in \(z\), which is subsequently modeled as a function of C-rate by the latent-space GP.

% At the output, we separate voltage-like channels from derivative-based channels because they are normalized differently during preprocessing. Charge and discharge voltage channels are min--max normalized to \([0,1]\) and are produced by a dedicated bounded head (sigmoid activation), whereas derivative-based channels (e.g., \(dV/dQ\), \(d^2V/dQ^2\), and \(dQ/dV\)) are z-score normalized and are produced by an unbounded linear head. This separation avoids imposing voltage-range constraints on derivative outputs and improves numerical stability during training.

% Finally, the capacity-coordinate channel \(q\) (or \(q_{\mathrm{cap}}\)) is used only as an input to the decoder and is \emph{not} reconstructed as part of the output target. Reconstructing \(q\) would be both redundant and potentially harmful in later-life cycles, where shortened CC segments lead to masked regions near the end of the grid: a deterministic coordinate channel would force the decoder to emit values in regions that are physically undefined and subsequently masked. Excluding \(q\) from the reconstruction target ensures that the decoder focuses its capacity on reconstructing the physically meaningful voltage-derived channels, while masking continues to handle variable support across cycles.

% \paragraph{Training objective and optimization.}
% The VAE is trained by minimizing the masked \(\beta\)-VAE objective (Section~\ref{sec:vae}), consisting of a reconstruction term and a KL regularizer. Reconstruction is computed only on valid regions of the capacity grid using the per-channel masks \(m\), such that padded/undefined values introduced by shortened CC segments do not contribute to the loss:
% \begin{equation}
% \mathcal{L}_{\mathrm{rec}}(x)=\big\lVert m \odot (x-\hat{x}) \big\rVert_2^2,
% \end{equation}
% and the KL term is computed in closed form for the diagonal-Gaussian posterior. The total loss is
% \begin{equation}
% \mathcal{L}(x)=\mathcal{L}_{\mathrm{rec}}(x)+\beta(t)\,\mathrm{KL}\!\left(q_\phi(z\mid x)\,\|\,p(z)\right),
% \end{equation}
% where \(\beta(t)\) is annealed during training to stabilize optimization and mitigate posterior collapse.

% We apply cosine annealing to \(\beta(t)\) over the first 20 epochs, with a maximum KL weight \(\beta_{\max}=10^{-4}\). Optimization uses Adam with batch size 64. The learning rate is initialized at \(10^{-3}\) and adapted using ReduceLROnPlateau with patience 20. Training is terminated using early stopping with patience 30 epochs and minimum improvement \(\Delta_{\min}=0.01\), selecting the checkpoint with the lowest validation loss.

% The latent dimensionality was set to \(d=2\). This choice is supported empirically by inspection of the per-dimension KL contributions: only two latent coordinates consistently exhibit non-zero KL, while additional dimensions collapse toward the prior (posterior collapse), indicating that they are not utilized by the model under the present dataset and objective.

%%%%%

\subsection{Why early cycles must be emphasized}
\label{sec:early_weight}
Although trajectories extend to 5000 cycles, the magnitude of change is not uniform over life:
the strongest curvature and feature evolution occurs in the early-to-mid regime, whereas later cycles exhibit comparatively
small incremental changes.
Training on uniformly sampled cycles therefore over-represents late-life near-redundant samples and can bias the model
toward minimizing errors where the signal is weakest.
To address this, we apply non-uniform importance over cycle index (or equivalently, resample cycles on a log-spaced grid).
Figure~\ref{fig:cycle_weights} visualizes the weighting (or sampling density) used in training.
In ablations, emphasizing early cycles improves reconstruction of derivative-sensitive channels and stabilizes the latent-space
organization reported below.

\subsection{VAE reconstruction and effective latent dimensionality}
\label{sec:vae_recon_kl}
We next evaluate whether the VAE captures cycle-level signatures in a compact latent representation.
Figure~\ref{fig:recon_examples} shows representative reconstructions for (i) voltage and (ii) derivative-based channels,
for both early and late cycles.
Reconstruction quality remains visually consistent across charge rates, including regimes where incremental-capacity-like
features are most structured.

To quantify the minimum latent complexity required to represent degradation trends, we track the KL contribution during
training and evaluate latent collapse.
Figure~\ref{fig:kl_sweep} reports the KL divergence versus epoch and (optionally) versus latent dimensionality.
We find that a total KL of approximately $\sim 2$ (and an effective dimensionality of two active latent components)
is sufficient to capture the dominant modes of trajectory variation; additional latent dimensions contribute near-zero KL,
indicating posterior collapse and limited additional explanatory power for this dataset.

\subsection{Latent space organizes aging progression and charge-rate variation}
\label{sec:latent_structure}
We analyze the learned embeddings using the encoder posterior mean $\mu_\phi(x)$.
Figure~\ref{fig:latent_space} visualizes the latent codes colored by (a) cycle index and (b) charge C-rate.
Two consistent structures emerge: (i) within each C-rate, cycles progress smoothly through latent space, forming a coherent
aging trajectory; and (ii) across C-rates, trajectories are systematically displaced, indicating that the latent representation
captures protocol-driven variation in addition to within-protocol degradation.
Importantly, we treat this structure as empirical organization rather than a direct mechanistic decomposition:
latent axes are not assigned physical meaning unless validated by targeted correlations to known degradation indicators.

\subsection{Gaussian-process surrogate in latent space: convergence and interpolation}
\label{sec:gp_latent}
We then fit a Gaussian-process (GP) surrogate in latent space to enable prediction at unseen charge rates.
Figure~\ref{fig:gp_convergence} shows the GP marginal log-likelihood (or loss) convergence and the learned kernel
length-scales, confirming stable optimization and smooth dependence on operating conditions.

For interpolation, we query the GP at held-out charge rates and decode the predicted latent distribution through the VAE decoder.
Figure~\ref{fig:interp_traj} compares predicted trajectories against PyBaMM ground truth for representative held-out rates,
shown for both early and late cycles.
The decoded predictions preserve the main voltage-shape evolution and derivative features while remaining smooth across
charge rate, demonstrating that regression in latent space is an effective low-dimensional surrogate for the full trajectory.

\subsection{Uncertainty on totally unseen test conditions}
\label{sec:uncertainty}
Finally, we evaluate uncertainty on held-out charge rates by sampling from the GP predictive distribution in latent space and
decoding an ensemble of trajectories.
Figure~\ref{fig:uncertainty_bands} shows pointwise predictive intervals for representative channels.
Uncertainty increases away from training-supported C-rates, as expected for epistemic uncertainty.

We assess calibration by empirical coverage of nominal intervals on held-out test data
(e.g., 90\% and 95\% bands).
Figure~\ref{fig:calibration} reports coverage (and interval width) versus distance to the nearest training rate,
highlighting the expected trade-off: tighter bands near observed regimes and wider, more conservative uncertainty as the model
moves into less-supported regions.


\paragraph{Encoder.}
Each cycle is represented by nine physically motivated channels: \(V_{\mathrm{ch}},V_{\mathrm{dis}}\); \(dV_{\mathrm{ch}}/dQ,dV_{\mathrm{dis}}/dQ\); \(d^2V_{\mathrm{ch}}/dQ^2,d^2V_{\mathrm{dis}}/dQ^2\); \((dQ/dV)_{\mathrm{ch}},(dQ/dV)_{\mathrm{dis}}\); and hysteresis \(H\). The capacity coordinate \(q\) is included as an input channel and further expanded using four Fourier features to increase representational capacity for fine-scale structure, resulting in 13 input channels per token. The concatenated sequence is linearly projected to token embeddings and processed by a lightweight Transformer encoder \cite{vaswani2017attention} with two self-attention layers. Each layer is conditioned on C-rate via FiLM \cite{perez2018film}, and validity masks are applied to exclude invalid regions from attention. The Transformer output is pooled using attention-based pooling \cite{ilse2018attention} and projected to \(\mu_\phi(x)\) and \(\log\sigma_\phi^2(x)\).

\paragraph{Decoder}
The decoder is implemented as a residual neural field over the capacity coordinate. Given Fourier features of the capacity grid $\phi(q) \in \mathcal{R}^{N \times F}$, the model predicts per-grid output as
\begin{equation}
    y(q,z,c) = f_{base}(\phi(q)) + f_{res}(\phi(q), z, c)
\end{equation}
where the baseline branch $\mathcal{f}_{base}$ depends only on $\phi(q)$, and the residual branch $\mathcal{f}_{res}$ conditions on the latent code $z$ (broadcast to all $N$ grid points). The residual branch first applies a linear projection and then a stack of pre-norm residula MLP block (RMSNorm $\rightarrow$ SiLU MLP $\rightarrow$ skip connection). No self-attention is used; the "Transformer-style" aspect is limited to the pre-norm residual block structure rather than attention-based token mixing. The output heads are split by normalization type: voltage-like channels are passed through a sigmoid to enforce $[0,1]$, while derivatives-based channels are produced by an ubbounded linear head. The capacity coordinate $q$ is treated as deterministic and is not reconstructed; in late-life cycle, 


% The decoder is intentionally lightweight to prevent it from ignoring the latent variable and reconstructing purely from coordinate information. For each sample, \(z\) is broadcast across the \(N\) grid points and concatenated with the Fourier features of \(q\). A linear projection followed by a shallow stack of MLP blocks produces per-token hidden features that are mapped to reconstructed channels. Voltage channels (min--max normalized to \([0,1]\)) are produced by a bounded head (sigmoid), while derivative-based channels (z-score normalized) are produced by an unbounded linear head. The capacity-coordinate channel is not reconstructed: \(q\) is deterministic and, in late-life cycles, portions of the grid are masked due to shortened CC segments; forcing the decoder to reproduce \(q\) would add a redundant constraint in physically undefined regions and is therefore avoided.

% \subsection{GP regression in latent space}\label{sec:gp}
% To generalize across operating conditions and quantify uncertainty at unseen charging rates, we perform regression in the learned latent space. For each cycle trajectory \(x\) at charge rate \(r\), we use the encoder posterior mean \(y=\mu_\phi(x)\in\mathbb{R}^d\) as the latent target and model each latent dimension \(y_j\) with a Gaussian process (GP):
% \begin{equation}
% f_j(r)\sim\mathcal{GP}(0,k_j(r,r')), \qquad y_j=f_j(r)+\epsilon_j.
% \end{equation}
% We use a stationary covariance kernel such as the RBF kernel,
% \begin{equation}
% k_{\mathrm{RBF}}(r,r')=\sigma_f^2\exp\!\left(-\frac{(r-r')^2}{2\ell^2}\right),
% \end{equation}
% with hyperparameters learned by maximizing the GP marginal log-likelihood. For an unseen rate \(r_\star\), the GP yields a predictive distribution \(p(y_\star\mid r_\star,\mathcal{D})=\mathcal{N}(\mu_\star,\Sigma_\star)\).
% Uncertainty is propagated to trajectory space by sampling \(z_\star\sim\mathcal{N}(\mu_\star,\Sigma_\star)\) and decoding \(\hat{x}_\star=g_\theta(z_\star)\), producing predictive intervals for each channel.
% Optionally, encoder uncertainty can be incorporated as input-dependent observation noise using the posterior variances \(\sigma_\phi^2(x)\) when fitting the GP.



% &&&&&&&&&&&
% After training the VAE, we freeze the encoder--decoder parameters and compute a latent embedding for every (cycle, C-rate) pair using the encoder posterior mean $\mu_\phi(x)$. We then fit Gaussian-process (GP) regressors that map operating conditions to the latent representation, enabling continuous interpolation in C-rate while preserving the low-dimensional structure learned by the VAE. In all experiments, generalization is evaluated using a leave-one-C-rate-out protocol: for each held-out charge rate $r_\star$, the GP is trained on latent embeddings from the remaining rates and queried at $r_\star$ across the full cycle range. Predicted latent distributions are decoded through the fixed VAE decoder to obtain predicted multi-channel trajectories $\hat{x}_\star$.

% \begin{figure}[!ht]
%   \centering
%   \includegraphics[width=\textwidth]{figures/GP/fold_performance_metrics.png}
%   \caption{Leave-one-C-rate-out evaluation of latent-space GP surrogate. Bars report (a) RMSE, and (b) test negative
% log-likelihood aggregated over all cycles for the held-out rate after decoding latent predictions through the VAE. Errors
% are smallest for interior rates and increase toward the boundaries of the simulated rate range.}
%   \label{fig:coverage_by_rate}
% \end{figure}

% Figure~\ref{fig:gp_metrics_by_rate} summarizes predictive performance as a function of the held-out rate.
% Errors (RMSE and MAE aggregated over the reconstructed channels and capacity grid) are lowest for interior rates
% (approximately $0.60$--$0.85$C) and increase toward the edges of the simulated rate range ($0.20$C and $1.00$C),
% consistent with the reduced local support available for interpolation at the boundaries.
% Interestingly, a marked degradation in calibration/performance is also observed at $0.50$C despite being an interior rate,
% suggesting that the mapping from C-rate to latent codes is not globally stationary and may exhibit localized curvature
% that is not fully captured by the GP kernel choice. This motivates the uncertainty analysis below and provides a concrete
% target for future improvements (e.g., non-stationary or rate-warped kernels).

% \subsection{Uncertainty propagation and calibration at unseen rates}
% \label{sec:gp_calibration}

% Uncertainty is obtained from the GP predictive distribution in latent space and propagated to trajectory space by sampling
% latent codes $z_\star \sim \mathcal{N}(\mu_\star,\Sigma_\star)$ and decoding each sample through the VAE.
% This yields an ensemble of reconstructed trajectories from which pointwise predictive intervals are computed for each
% channel on the capacity grid. We evaluate calibration via empirical coverage of nominal predictive intervals on the held-out
% rate:
% \begin{equation}
% \mathrm{Coverage}_\alpha=\frac{1}{|\mathcal{T}|}\sum_{(x,r)\in\mathcal{T}}
% \mathbb{I}\big[x \in \mathrm{PI}_\alpha(r)\big],
% \end{equation}
% where $\mathrm{PI}_\alpha(r)$ denotes the $\alpha$-level predictive interval and $\mathcal{T}$ is the test set at the
% held-out rate.

% \begin{figure}[!ht]
%   \centering
%   \includegraphics[width=\textwidth]{figures/GP/coverage_by_fold.png}
%   \caption{Calibration of predictive intervals under leave-one-C-rate-out evaluation. Empirical coverage of nominal 90\% and 95\% predictive intervals is shown for each held-out rate. Interior rates are near-nominal while low-rate regimes exhibit under-coverage, indicating underestimated uncertainty and/or systematic bias.}
%   \label{fig:coverage_by_rate}
% \end{figure}

% Figure~\ref{fig:coverage_by_rate} reports empirical coverage for 50\%, 90\% and 95\% intervals across held-out rates. Coverage is close to nominal (and in some cases slightly conservative) for interior rates, indicating that the GP posterior variance captures the dominant epistemic uncertainty when interpolating between well-supported training regimes. In contrast, under-coverage is observed for low-rate regimes (notably $0.20$C--$0.50$C), indicating that uncertainty is underestimated in those regions and that residual systematic error (bias) is not fully explained by the latent-space GP variance alone. Consistent with epistemic expectations, predictive interval widths increase toward the boundaries of the rate range (Figure~\ref{fig:pi_width_by_rate}), but wider intervals are still insufficient to fully calibrate the lowest-rate
% held-out cases.

% To diagnose where miscalibration concentrates over life, Supplementary Figures~S\ref{fig:cov_cycle_bins}--S\ref{fig:err_cycle_bins} report coverage and absolute error binned by cycle index. These results show that calibration can vary substantially with cycle regime, supporting the use of cycle-resolved evaluation rather than a single aggregated coverage score.


% \subsection{Generalization to unseen C-rate (GP in latent space)}
% We next evaluate whether GP regression in the learned latent space enables accurate prediction at unseen charging rates. The GP is trained on latent embeddings from the training C-rates and queried at held-out rates \(r_\star\). Predicted latent distributions \(p(z_\star \mid r_\star)\) are decoded to obtain predicted trajectories \(\hat{x}_\star\). Performance is assessed by comparing predicted trajectories against the corresponding PyBaMM-generated ground truth at the held-out rates.

% \textbf{Figure~\ref{fig:unseen_rate_predictions}} compares predicted and ground-truth trajectories for representative held-out C-rates, including both early and late-cycle regimes. We report quantitative errors aggregated over the held-out set (e.g., masked RMSE over all channels, and end-of-life capacity error if capacity is derived consistently from the trajectories). To contextualize gains, we compare against baselines that regress directly in observation space or interpolate per-channel features across C-rate (details in Section~\ref{sec:evaluation}). Results indicate that latent-space regression yields improved accuracy and stability, particularly for derived channels that are sensitive to noise and nonlinearity.

% % Needed: unseen C-rate prediction figure (multiple rates, multiple cycles)
% % Needed: table of errors vs baselines

% \subsection{Uncertainty calibration}
% Finally, we assess whether the proposed approach produces meaningful and calibrated uncertainty estimates at unseen charging rates. Uncertainty arises from the GP predictive distribution in latent space and is propagated through the decoder by sampling latent codes and reconstructing an ensemble of trajectories. From this ensemble, we compute pointwise predictive intervals for each channel on the capacity grid.

% Calibration is evaluated using empirical coverage of nominal predictive intervals (e.g., 90\% and 95\%) on the held-out C-rates:
% \begin{equation}
% \mathrm{Coverage}_\alpha = \frac{1}{|\mathcal{T}|}\sum_{(x,r)\in \mathcal{T}} \mathbb{I}\left[x \in \mathrm{PI}_\alpha(r)\right],
% \end{equation}
% where \(\mathrm{PI}_\alpha(r)\) denotes the \(\alpha\)-level predictive interval and \(\mathcal{T}\) is the test set. \textbf{Figure~\ref{fig:calibration}} reports coverage versus nominal level and shows that predictive intervals widen as the queried C-rate moves away from the nearest training rates, consistent with epistemic uncertainty. We also report interval widths as a function of distance to the training set to verify that the method expresses greater uncertainty in extrapolation-like regimes.

% Needed: calibration plot (nominal vs empirical coverage)
% Needed: example trajectories with uncertainty bands
% Optional: interval width vs distance to nearest train rate

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Minimal figure/table checklist (so Results doesn’t feel incomplete)
%   1. Table 1: dataset summary + split.
%   2. Fig 1: example preprocessed channels (early/late, low/high C-rate).
%   3. Fig 2: reconstructions (GT vs recon).
%   4. Table 2: reconstruction metrics (+ ablations optional).
%   5. Fig 3: latent visualization (UMAP/PCA).
%   6. Fig 4: unseen-rate predictions (GT vs mean, multiple cycles).
%   7. Table 3: unseen-rate errors vs baselines.
%   8. Fig 5: uncertainty calibration (coverage + example bands).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


